Better Membership Inference Privacy Measurement through Discrepancy

Membership Inference Attacks have emerged as a dominant method for empirically measuring privacy leakage from machine learning models. Here, privacy is measured by the {\em{advantage}} or gap between a score or a function computed on the training and the test data. A major barrier to the practical deployment of these attacks is that they do not scale to large well-generalized models -- either the advantage is relatively low, or the attack involves training multiple models which is highly compute-intensive. In this work, inspired by discrepancy theory, we propose a new empirical privacy metric that is an upper bound on the advantage of a family of membership inference attacks. We show that this metric does not involve training multiple models, can be applied to large Imagenet classification models in-the-wild, and has higher advantage than existing metrics on models trained with more recent and sophisticated training recipes. Motivated by our empirical results, we also propose new membership inference attacks tailored to these training losses.

==> sections/Discrepancy.tex <==
\section{Discrepancy: An Upper Bound on Advantage}

%0: lower bound of advantage. motivates the upper bound. discuss the meaning of the upper bound.
%1: draw the connection to the discrepancy distance and propose the upper bound.
%2: Choose a family -- convex family; Prove 4 probability-based scores are in this family.
%3: Introduce how to approximately compute this upper bound.
While many prior works have been making many towards better MIAs in terms of higher advantage, the upper bound of the advantage among a family of MIAs hasn't gotten much attention yet.
The upper bound can be useful for two reasons: 1. it is a stronger privacy metric than any single MIA in this family; 2. the comparison between the upper bound and the existing MIAs in the family indicates how good these MIAs are, which can motivate the better design of MIA potentially.
In this paper, we focus on MIAs which threshold the probability-based scores and we particularly study a family of scores that are convex in $(f(x), y)$. 
We first show that all four common probability-based scores, as reviewed in Section~\ref{sec:preliminary}, either are in this family or agree on a score in this famil.
As a consequence, the advantages of all four common probability-based scores with arbitrary thresholds are bounded by the upper bound over this family.



Many statistics have been proposed to answer the question of how much membership information the model may leak \cite{ yeom2018privacy, song2020systematic}. The advantage of these statistics can be viewed as lower bound of privacy leakage for a given model. For example, the MIA proposed by \cite{yeom2018privacy} yields that the generalization gap is an lower bound of privacy leakage, i.e. the larger the generalization gap, the more likely the MIA succeed.
 
In this paper, we propose a new statistics that can be viewed as upper bound of a family of statistics. First of all, we consider the advantage of adversary from the perspectives of discrepancy distance between training samples and test distribution. 
% We look at a family of statistics and derive an upper bound of membership leakage with respect to this family of statistics. \\
For a MIA $\mathcal{A}$, we denote the discriminative set of $\mathcal{A}$ as $Q(\mathcal{A}) = \{(f(\bx),\by) \text{ s.t. } \mathcal{A}(z,f) = 1\}$, when the context is clear, we write it as $Q$.
% and $Q_0(\mathcal{A}) = \{z \text{ s.t. } \mathcal{A}(z,f) = 0\}$
The following theorem states that for a family of MIA, the discrepancy distance between training samples and test distribution over the corresponding discriminative set is an upper bound to the greatest advantage, i.e. strongest attack. 
\begin{theorem}
    Consider a family of attack $A$, and the set of discriminative set $\mathcal{Q} = \{ Q(\mathcal{A}), \forall \mathcal{A} \in A \}$ . Then
    \begin{equation}
        \sup_{\mathcal{A}\in A} Adv(\mathcal{A},f, S,\mathcal{D}) \leq \sup_{Q \in \mathcal{Q}}|\mathbb{P}_{z \sim S}[(f(\bx),\by) \in Q] - \mathbb{P}_{z \sim \mathcal{D}}[(f(\bx),\by) \in Q]|
    \end{equation}
    \end{theorem}
    \begin{proof}
    By second definition of advantage \ref{advatage_df2}, we have 
        \begin{align*}
            \sup_{\mathcal{A}\in A} Adv(\mathcal{A}, f, S, \mathcal{D}) & = \sup_{\mathcal{A}\in A}\mathbb{P}(\mathcal{A}(z,f) = 1|b=1) - \mathbb{P}(\mathcal{A}(z,f) = 1|b=0) \\
            & = \sup_{\mathcal{A}\in A} \mathbb{P}_{z\sim S}[(f(\bx),\by)\in Q(\mathcal{A})] - \mathbb{P}_{z\sim \mathcal{D}}[(f(\bx),\by) \in Q(A)] \\
            & \leq \sup_{Q \in Q}|\mathbb{P}_{z\sim S}[(f(\bx),\by)\in Q] - \mathbb{P}_{z\sim \mathcal{D}}[(f(\bx),\by) \in Q]| \tag*{\qedhere}
        \end{align*}
    \end{proof} 
Since $Q$ characterize an attack $\mathcal{A}$, we may discuss the family of attack using the family of $\mathcal{Q}$.
Hence, the goal of our paper is to estimate $$\sup_{Q \in \mathcal{Q}}|\mathbb{P}_{z \sim S}[(f(\bx),\by) \in Q] - \mathbb{P}_{z \sim \mathcal{D}}[(f(\bx),\by) \in Q]|$$ for some suitable $\mathcal{Q}$.
Note that the choice of $\mathcal{Q}$ can be considered as the power of the adversary. If we choose $\mathcal{Q}$ to be any subset of $\mathbb{R}^{2C}$, then the advantage is 1, since we can simply let $Q = S$. In this case, the analysis is not interesting, and we may not assume the adversary have the entire knowledge of the exact training sample. Hence, we need to add some constraint to the adversary. In this paper, we choose $\mathcal{Q}$ to be all the convex set.
\subsection{Convex Family}
% \paragraph{Choosing the convex family.}
%Existing MIs are equivalent to a convex or concave discriminative set.
In this section, we show that the convex family is a suitable subset of statistics for the discrepancy distance and several common statistics is included in this convex family. We start by introducing 4 popular existing MI statistics:

Denote the number of class as $C$ and the logit as $\bp = f(\bx) \in \mathbb{R}^C$, 
\begin{itemize}%[noitemsep, leftmargin=*, topsep=0pt]
	\item Max-softmax-probability (MSP): $m_{\rm MSP}(\bp, \by; \tau)=\mathds{1}\left[\max_{c\in [C]}\bp_c > \tau\right]$;
	\item Entropy (ENT): $m_{\rm ENT}(\bp, \by; \tau)=\mathds{1}\left[\sum_{c\in [C]}-\bp_c\log(\bp_c) < \tau\right]$;
	\item Cross-entropy loss (CE): $m_{\rm CE}(\bp, \by; \tau)=\mathds{1}\left[\sum_{c\in [C]}-\by_c\log(\bp_c) < \tau\right];$
	\item Modified-entropy (ME):\\ 
	$m_{\rm ME}(\bp, \by; \tau)=\mathds{1}\left[-\sum_{c\in [C]}\left((1-\bp_c)\log(\bp_c)\by_c + \bp_{c}\log(1-\bp_{c})(1-\by_c)\right)<\tau\right].$
\end{itemize}
We show that these four MI statistics is equivalent to an MI induced by a convex or concave subset of $\mathbb{R}^{2C}$. To formally state it in the following theorem, we first introduce some notations. For two functions $F, F':\calV\to \bbR$ and $\calV^*\subset\calV$, we say $F\equiv_{\calV^*} F'$ if $\forall \bv\in \calV^*,F(\bv)= F'(\bv)$. Define $\calV^*:=\{(\theta(\bx), \by)| (\bx, \by) \in S\cup D_{\rm test}\}$.
\begin{lemma}
\label{thm:cvx_dscrm}
$\forall m\in\{m_{\rm MSP}, m_{\rm ENT}, m_{\rm CE},m_{\rm ME}\}$ and $\tau$, there exists a convex or concave set $Q\subseteq (0, 1]^C \times [0, 1]^C$ s.t. $MI_{Q}\equiv_{\calV^*}m(\bp, \by)$.
\end{lemma}
The proof of the lemma is included in Appendix. We highlight this result since even though CE and ME are non-convex in $(\bp, \by)$, the discriminative set is still in the convex family. 
\begin{corollary}
	There exists an $F(\bp, \by)$ s.t. 
	\begin{enumerate}
	\item $F(\bp, \by)$ is not convex or concave on $(0, 1]^C \times [0, 1]^C$.
	\item We can still find a such a convex or concave $Q\subseteq (0, 1]^C \times [0, 1]^C$ under which $MI_{Q}(\bp, \by)\equiv_{\calV^*}\mathds{1}\left[F(\bp, \by)<\tau\right]$.
	\end{enumerate}
\end{corollary}
\begin{proof}
	$F(\bp, \by)=\sum_{c\in [C]}-\by_c\log(\bp_c)$ is not convex and as shown in Lemma~\ref{thm:cvx_dscrm} there exists a $Q$.
\end{proof}
Hence, the discrepancy distance with respect to the convex family is an upper bound to all four statistics, which can be formally stated in the following theorem.
\begin{theorem}
	The advantage of $m_{\rm MSP}, m_{\rm ENT}, m_{\rm CE},m_{\rm ME}$ is bounded by the discrepancy distance between $S$ and $\mathcal{D}$ over a family $\calQ_{cvx}$ of convex subsets of $\bbR^{2C}$. In the other word, $\forall m\in\{m_{\rm MSP}, m_{\rm ENT}, m_{\rm CE},m_{\rm ME}\}$,
	$$
	Adv(m, f, S, \mathcal{D})\leq \sup_{Q\in \calQ_{cvx}}\left|\bbP_{(\bx, \by)\sim S}\left((f(\bx), \by)\in Q\right) - \bbP_{(\bx, \by)\sim D_{\rm test}}\left((f(\bx), \by)\in Q\right)\right|.
	$$
\end{theorem}
\begin{proof}
$\forall m\in\{m_{\rm MSP}, m_{\rm ENT}, m_{\rm CE},m_{\rm ME}\}$,
\ref{thm:cvx_dscrm} shows that $\exists$ a convex or concave $Q_m \subseteq (0.1]^C \times [0,1]^C$ s.t. $MI_{Q_m} \equiv_{\calV^*} m(\bp, \by)$, then
\begin{align*}
    Adv(m, f, S, \mathcal{D}) & = \bbP_{(\bx, \by)\sim S}\left((f(\bx), \by)\in Q_m\right) - \bbP_{(\bx, \by)\sim \mathcal{D}}\left((f(\bx), \by)\in Q_m\right) \\
    & \leq \sup_{Q\in \calQ_{cvx}}\left|\bbP_{(\bx, \by)\sim S}\left((f(\bx), \by)\in Q\right) - \bbP_{(\bx, \by)\sim D_{\rm test}}\left((f(\bx), \by)\in Q\right)\right|
\end{align*}
Since $Q_m \in \mathcal{Q}_{cvs}$.
    
\end{proof}
\subsection{Convex Polytope Bound and Convex Polytope Machine}
In this section, we show how to estimate
\begin{equation}\label{convexset-def}
    \sup_{Q\in \calQ_{cvx}}\left|\bbP_{(\bx, \by)\sim S}\left((f(\bx), \by)\in Q\right) - \bbP_{(\bx, \by)\sim \mathcal{D}}\left((f(\bx), \by)\in Q\right)\right|
\end{equation}
The first result comes from the theorem that every convex bodies can be approximate by k-polygons as k goes to infinity \cite{gruber1982approximation}. Several Euclidean geometry articles have proved the following results \cite{bronshteyn1975approximation}:
\begin{theorem}
For a convex body $C \in \mathbb{R}^d$, denote $\delta$ as the Hausdorff-metric, and $\mathcal{P}_k$ as all polytopes having at most $k$ vertices, then
    $$\delta(C, \mathcal{P}_k) \leq \frac{constant}{k^{2/(d-1)}}, \forall k \in \mathbb{N}$$
where $\delta(C, \mathcal{P}_k) = \inf \{\delta(C, P)| P \in \mathcal{P}_k \}$
\end{theorem}
Hence, as $k$ tends to infinity, we can approximate any convex function using k-convex polytope. Therefore, \ref{convexset-def} is equivalent to 
\begin{equation}\label{convex-polygon-def}
    \sup_{Q\in \mathcal{P}_k}\left|\bbP_{(\bx, \by)\sim S}\left((f(\bx), \by)\in Q\right) - \bbP_{(\bx, \by)\sim \mathcal{D}}\left((f(\bx), \by)\in Q\right)\right|, \text{ as }k \to \infty
\end{equation}
We denote \ref{convex-polygon-def} as Convex Polytope Bound (CPB). To estimate the CPB, we uses Convex Polytope Machine (CPM) methods proposed by \cite{kantchelian2014large}. We treat this as a supervised binary classification problem that aims to find a good classifier $c: \mathbb{R}^{2C} \to \{-1,1 \}$ such that $c(f(\bx),y) = 1$, if $(\bx,\by) \in S$, -1 otherwise. Using the first definition of advantage \ref{advatage_df1}, we have that 
$$\arg \max_{c\in \mathcal{P}_K} 2 \bbE[c(f(\bx),\by) = b] - 1 \equiv \arg \max_{c \in \mathcal{P}_K} \mathbb{E}[c(f(\bx),\by)=b]$$
and the convex polytope can be modeled as $$\mathcal{P}_K = \{g:\mathbb{R}^{2C} \to \mathbb{R}| g(\bx) = \max_{1\leq c\leq C} (\textbf{W}\bx)_c,  \textbf{W} \in \mathbb{R}^{K\times C}\}$$ and for each $g$ it induced a classifier $c_g$ such that $c_g(z) = 1$ if $g(z) \geq 0$, and $c_g(z) = 0$ if $g(z) < 0$. It can be solved using a soft-SVM like method with objective function:
\begin{align*}
    & \min_{W,\epsilon} ||W||^2 + C\sum_{i = 1}^n \epsilon_i \\
     \text{subject to }    \forall i: & y^{(i)} = -1,  y^{(i)}W_kx^{(i)} \geq 1-\epsilon_i, \forall k \in \{ 1,...,K\}\\
    & y^{(i)} = 1, y^{(i)}W_{z(x^{(i)})}x^{(i)} \geq 1-\epsilon_i
\end{align*}



==> sections/checklist.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count , towards the page limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: in the introduction and abstract, we accurately demonstrate the main paper's theoretical results and observations from experiment results. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the limitations of the work in the section \ref{sec:Conclusion}. For example, we discuss the limitation of only considering the convex family of statistics, and some future work can consider a larger family of statistics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: For our theoretical results, we have included a complete detailed proof in Appendix \ref{sec:appendix} and a sketch of the proof in the main paper. We have referenced every theorem we use in the proof and stated all the assumptions we have made. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our experiment results are easily reproducible. We have introduced our algorithm in section \ref{sec:approximation of the discrepancy}, which can be implemented using PyTorch package. Moreover, in section \ref{Sec:Experiment}, we include all the training details.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We use public datasets, including CIFAR, ImageNet and MNIST datasets, and can be accessed by everyone. We have provided sufficient instructions to reproduce the experimental results in the paper and we will release the code when it is published. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have included all the training and test details in \ref{Sec:Experiment}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The algorithm we propose is to evaluate the privacy leakage of individual trained model, instead of the training algorithm. We report the test accuracy of each trained models and they are trained with adequate performance.  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have included this details in Section \ref{Sec:Experiment}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have follow the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    % the topic discussed in this paper aims to evaluate the privacy leakage of machine learning models. 
    The method proposed in this paper can be used to audit the privacy leakage of publicly released large machine-learning models. It does not involve malicious uses since the adversary does not obtain the entire training sample. 
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper poses no such risks
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have cited the model owner, data owner, etc.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not release new assets
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> sections/discrepancy_ruihansnotes.tex <==
\section{Proofs of Theorems in Section~\ref{sec:discrepancy}}
\subsection{Proof of Theorem~\ref{thm:cvx_dis_up}}
\begin{proof}[Proof of Theorem~\ref{thm:cvx_dis_up}.]
For $m_{\rm MSP}$, because $\max_{c\in [C]}\bp_c$ is convex in $(\bp, \by)$ when $(\bp, \by)\in \bbR^{2C}$, from the convex property, $\left\{(\bp, \by, \tau)|\max_{c\in [C]}\bp_c\leq \tau, (\bp, \by, \tau)\in \bbR^{2C+1}\right\}$ is a convex set. Consequently, for a specific $\tau$, $\left\{(\bp, \by)|\max_{c\in [C]}\bp_c\leq \tau, (\bp, \by)\in \bbR^{2C}\right\}$ is a convex set. We can then define $Q$ as $\left\{(\bp, \by)|\max_{c\in [C]}\bp_c\leq \tau, (\bp, \by)\in \bbR^{2C}\right\}$ and it is easy to check the correctness that $MI_{Q}\equiv m(\bp, \by)$ for $(\bp, \by)$ in $(0,1]^C \times \{0,1\}^C$. Following the same argument, we can prove this for $m_{\rm ENT}$.

For $m_{\rm CE}$, it takes more effort, because $\sum_{c\in [C]}-\by_c\log(\bp_c)$ is no longer convex in $(\bp, \by)$. 
We will construct a $\tilde{m}(\bp, \by)=\mathds{1}\left[F(\bp, \by)< \tau\right]$ for $(\bp, \by)\in (0, 1]^C \times [0, 1]^C$, which has the following property:
\begin{enumerate}
\item $F(\bp, \by)= \sum_{c\in [C]}-\by_c\log(\bp_c)$, for $(\bp, \by)$ in $(0,1]^C \times \{0,1\}^C$.
% i.e. for all $(\bp, \by)\in\{(\theta(\bx), \by)| (\bx, \by) \in S\cup D_{\rm test}\}$, $F(\bp, \by)=\sum_{c\in [C]}-\by_c\log(\bp_c)$
\item $F(\bp, \by)$ is a convex function of $(\bp, \by)$ on $(0, 1]^C \times [0, 1]^C$.
\end{enumerate}
If such $\tilde{m}$ exists, because of the second property, by following the same argument for $m_{\rm MSP}$, we can prove there exists a convex set $Q\subseteq \bbR^{2C}$ s.t. $MI_{Q}(\bp, \by)=\tilde{m}(\bp, \by)$ for all $(\bp, \by)\in\{(\theta(\bx), \by)| (\bx, \by) \in S\cup D_{\rm test}\}$. 
Moreover, property 1 implies that $m(\bp, \by)=\tilde{m}(\bp, \by)$ for all $(\bp, \by)\in\{(\theta(\bx), \by)| (\bx, \by) \in S\cup D_{\rm test}\}$, which completes the proof.

Now we are going to show the construction of $\tilde{m}=\mathds{1}\left[F(\bp, \by)< \tau\right]$. 
We define
$$
F(\bp, \by):=\sum_{c\in [C]}-\by_c\log(\bp_c) + \sum_{c: \by_c\neq 0} \by_c\log(\by_c), \forall(\bp, \by)\in (0, 1]^C \times [0, 1]^C.
$$
By definition, property 1 naturally holds. We are going to verify the property 2.
Firstly, $F(\bp, \by)$ is a continuous function on $(0, 1]^C \times [0, 1]^C$ by the fact that $\lim_{a\to 0}a\log(a)=0$.
Secondly, we can prove $\nabla^2_{\bp, \by}F(\bp, \by)\succeq \mathbf{0}\ \forall(\bp, \by)\in (0, 1]^C \times {\color{red}(}0, 1]^C$.
It is sufficient to prove $\nabla^2_{\bp_c, \by_c}F(\bp, \by)\succeq \mathbf{0}$ because $\nabla^2_{\bp_c, \by_{c'}}F(\bp, \by)= \mathbf{0}$ when $c\neq c'$.
To see $\nabla^2_{\bp_c, \by_c}F(\bp, \by)\succeq \mathbf{0}$, $\forall \ba\in \bbR^2$,
$$
\ba\nabla^2_{\bp_c, \by_c}F(\bp, \by)\ba^{\top} = \frac{\by_c}{\bp_c^2}\ba_1^2 - \frac{2}{\bp_c}\ba_1\ba_2 + \frac{1}{\by_c}\ba_2^2=\frac{1}{\by_c} \left(\frac{\by_c}{\bp_c}\ba_1-\ba_2\right)^2\geq 0.
$$
Therefore $F(\bp, \by)$ is a convex function of $(\bp, \by)$ on $(0, 1]^C \times [0, 1]^C$.

Similarly, for $m_{\rm ME}$, we are going to construct an $F$ such that 
\begin{enumerate}
\item $F(\bp, \by)=-\sum_{c\in [C]}\left((1-\bp_c)\log(\bp_c)\by_c + \bp_{c}\log(1-\bp_{c})(1-\by_c)\right)$ for $(\bp, \by)$ in $(0,1]^C \times \{0,1\}^C$.
\item $F(\bp, \by)$ is a convex function of $(\bp, \by)$ on $(0, 1]^C \times [0, 1]^C$.
\end{enumerate}
We define 
$$F(\bp, \by):=-\sum_{c\in [C]}\left((1-\bp_c)\log(\bp_c)\by_c + \bp_{c}\log(1-\bp_{c})(1-\by_c)\right)
$$
$$
+5\sum_{c: \by_c\neq 0} \by_c\log(\by_c) + 5\sum_{c: \by_c\neq 1} (1-\by_c)\log(1-\by_c).
$$

By definition, property 1 naturally holds. We are going to verify the property 2.
Firstly, $F(\bp, \by)$ is a continuous function on $(0, 1]^C \times [0, 1]^C$ by the fact that $\lim_{a\to 0}a\log(a)=0$.
Secondly, we can prove $\nabla^2_{\bp, \by}F(\bp, \by)\succeq \mathbf{0}\ \forall(\bp, \by)\in (0, 1]^C \times {\color{red}(}0, 1]^C$.
It is sufficient to prove $\nabla^2_{\bp_c, \by_c}F(\bp, \by)\succeq \mathbf{0}$ because $\nabla^2_{\bp_c, \by_{c'}}F(\bp, \by)= \mathbf{0}$ when $c\neq c'$.
To see $\nabla^2_{\bp_c, \by_c}F(\bp, \by)\succeq \mathbf{0}$, $\forall \ba\in \bbR^2$,

\begin{align*}
\ba\nabla^2_{\bp_c, \by_c}F(\bp, \by)\ba^{\top} &= \left(\by_c\cdot \left(\frac{1}{\bp_c^2} + \frac{1}{\bp_c}\right) + (1-\by_c)\cdot \left(\frac{1}{(1-\bp_c)^2} + \frac{1}{1-\bp_c}\right) \right)\ba_1^2\\
&+ 2 \left(\frac{1}{1-\bp_c}-\frac{1}{\bp_c}+\log(\bp_c)-\log(1-\bp_c)\right)\ba_1\ba_2+ \left(\frac{3}{\by_c} + \frac{3}{1-\by_c}\right)\ba_2^2\\
&= \frac{1}{\by_c}\left(\frac{\by_c}{\bp_c}\ba_1 - \ba_2\right)^2 
+ \frac{1}{1-\by_c}\left(\frac{1-\by_c}{1-\bp_c}\ba_1 - \ba_2\right)^2\\
&+\left(\frac{\by_c}{\bp_c}\ba_1^2 + 2\log(\bp_c)\ba_1\ba_2 + \frac{4}{\by_c}\ba_2^2\right)+\left(\frac{1-\by_c}{1-\bp_c}\ba_1^2 + 2\log(1-\bp_c)\ba_1\ba_2 + \frac{4}{1-\by_c}\ba_2^2\right)\\
&\geq \left(\frac{\by_c}{\bp_c}\ba_1^2 + 2\log(\bp_c)\ba_1\ba_2 + \frac{4}{\by_c}\ba_2^2\right)+\left(\frac{1-\by_c}{1-\bp_c}\ba_1^2 + 2\log(1-\bp_c)\ba_1\ba_2 + \frac{4}{1-\by_c}\ba_2^2\right)
\end{align*}
We are going to first prove $\frac{\by_c}{\bp_c}\ba_1^2 + 2\log(\bp_c)\ba_1\ba_2 + \frac{4}{\by_c}\ba_2^2\geq 0 $. Because $\frac{\by_c}{\bp_c}>0$, it is sufficient to prove
$(2\log(\bp_c))^2\leq 4\cdot \frac{\by_c}{\bp_c}\cdot \frac{4}{\by_c}$, which is equivalent to $-\log(\bp_c)\leq 2\sqrt{\frac{1}{\bp_c}}$. Define $h(\bp_c)=2\sqrt{\frac{1}{\bp_c}} +\log(\bp_c)$. $\forall \bp_c\in(0, 1]$, $h'(\bp_c)=-\frac{1}{\sqrt{\bp_c}\bp_c} +\frac{1}{\bp_c}<0$. Thus, $h(\bp_c)\geq h(1)=\sqrt{2}>0$ and $\frac{\by_c}{\bp_c}\ba_1^2 + 2\log(\bp_c)\ba_1\ba_2 + \frac{4}{\by_c}\ba_2^2\geq 0 $ has been proved. 

Similarly, we can prove $\left(\frac{1-\by_c}{1-\bp_c}\ba_1^2 + 2\log(1-\bp_c)\ba_1\ba_2 + \frac{4}{1-\by_c}\ba_2^2\right)\geq 0$ and we have completed the proof for $\ba\nabla^2_{\bp_c, \by_c}F(\bp, \by)\ba^{\top}\geq 0$. We now have the convexity of $F(\bp, \by)$  on $(0, 1]^C \times [0, 1]^C.$
\end{proof}

\subsection{Proof of Theorem~\ref{thm:cvx_up2}}
\begin{proof}[Proof of Theorem~\ref{thm:cvx_up2}]
\citet{niederreiter1972discrepancy} has proved an easier statement: $D_{\calQ_{cvx}}(S, \calD) = D_{\calQ_{cvx_poly}}(S, \calD)$,
where $\calQ_{cvx_poly}$ is a set of all convex polytopes.
The statement in this theorem is harder because $\calQ_{cvx, k}$ is a subset of $\calQ_{cvxpoly}$.

Similar to the proof in \citet{niederreiter1972discrepancy}, $\forall Q\in \calQ_{cvx}$, we are going to find $Q_1, Q_2\in \calQ_{cvx, k}$ such that $\bbP_{z\sim \calD}((f(x), y)\in Q_1)\leq \bbP_{z\sim S}((f(x), y)\in Q)\leq \bbP_{z\sim \calD}((f(x), y)\in Q_2)$ and $\bbP_{z\sim S}((f(x), y)\in Q)=\bbP_{z\sim \calD}((f(x), y)\in Q_1)=\bbP_{z\sim S}((f(x), y)\in Q_2)$.
Within this $Q_1, Q_2$, 
$$D(S, \calD|Q)\leq \max\{D(S, \calD|Q_1), D(S, \calD|Q_2)\},$$
and therefore $D_{\calQ_{cvx}}(S, \calD)\leq D_{\calQ_{cvx, k}}(S, \calD)$.
It is obvious that $D_{\calQ_{cvx}}(S, \calD)\geq D_{\calQ_{cvx, k}}(S, \calD)$ because $\calQ_{cvx, k}\subseteq \calQ_{cvx}$.
Thus $D_{\calQ_{cvx}}(S, \calD) = D_{\calQ_{cvx_poly}}(S, \calD)$.

To find $Q_1$, for any convex set $Q\in Q_{cvx}$, 
	if $Q\cap S=\emptyset$, we simply choose $Q_1\emptyset$.
	If $Q\cap S\neq\emptyset$, we can consider a convex hull $Q_1$ for $Q\cap S$.
	From the definition of the convex hull, $Q_1\subseteq Q$.
	In both two cases above,	$$
	\bbP_{z\sim S}((f(x), y)\in Q) - \bbP_{z\sim \calD}((f(x), y)\in Q) \leq \bbP_{z\sim S}((f(x), y)\in Q_1) - \bbP_{z\sim \calD}((f(x), y)\in Q_1)
	$$
	Because $Q\cap S$ is a discrete point set, the convex hull $Q_1$ would be a convex polytope whose vertices are a subset of $Q\cap S$.
	The Upper Bound Theorem~\citep{ziegler2012lectures} shows that the number of facets of a convex polytope with at most $|S|$ vertices can be bounded by $\binom{|S|}{2C}$, where $2C$ is the dimensionality of the space.
	
To find $Q_2$, we follow the proof in \citet{niederreiter1972discrepancy} to construct a $Q'$ first: if $Q$ is an open set, we set $Q':= Q$; otherwise we can enlarge $Q$ to $Q'$ such that the points in $Q\cap S$ are all the \emph{interior} points of $Q'$ but $Q'$ doesn't contain $S\backslash (Q\cap S)$.
Then for each $z\in S\backslash (Q\cap S)$, we can find a supporting hyperplane of $Q'$ such that $Q'$ lies in the closed halfspace $H_z$ defined by this supporting hyperplane.
Denote $H_z'$ as the corresponding open halfspace and define $Q_2:=H_z'\cap_{z\in S\backslash (Q\cap S)}$.
By definition, $\forall z\in S\backslash (Q\cap S)$, $z\notin Q_2$; $\forall z\in Q\cap S$, $z\in \mathrm{int}(Q)\subseteq \mathrm{int}(H_z\cap_{z\in S\backslash (Q\cap S)})=Q_2$, where $\mathrm{int}$ indicates the interior of a convex set.
Therefore, $\bbP_{z\sim S}((f(x), y)\in Q) = \bbP_{z\sim S}((f(x), y)\in Q_2)$.
Moreover, given the property of the data distribution $\calD$\ruihan{add one more assumption for $\calD$}, $\bbP_{z\sim \calD}((f(x), y)\in Q)= \bbP_{z\sim \calD}((f(x), y)\in \mathrm{int}(Q))\leq \bbP_{z\sim \calD}((f(x), y)\in Q_2)$.
Lastly, by the definition $Q_2$, it is an open convex polytopes with at most $|S|\leq \binom{|S|}{2C}$ facets.

\end{proof}

==> sections/upper_adv.tex <==
%\section{Study the Advantage Upper Bound over MIA Families}

\section{A Better Empirical Privacy Metric}

%Recall from Section X that the advantage of a MIA is an empirical measure of how private a model is, and different score-based MIAs provide measures on different datasets. This raises a natural question: can we find an empirical privacy metric that provides a more fine-grained 

Recall from Section~\ref{sec:preliminary} that the advantage of a MIA on a model $f$ is an empirical privacy metric that measures how much $f$ ``leaks'' its training data, and that different score-functions perform differently depending on the model and dataset. This raises a natural question: can we find an empirical privacy metric that encompasses all these scores-based advantages?

Before defining this better metric, we would like to discuss three properties that we expect from this metric. 
First, it should be an upper bound on the advantage of an entire class of score-based MIAs, ensuring that it is a reasonably {\em{strict}} privacy metric. 
Second, the metric should be able to distinguish between different models so that we can use it to compare models by their privacy leakage; in other words, the class of score-based MIAs should not be so expressive that training and test data can always be perfectly separated. 
Finally, it should be computable, or at the very least, approximately computable, with relative ease.  

%\begin{itemize}
%\item define upper bound over family
%\item $M_{cvx}$ --> what is this? why do we choose it? (a) covers many existing score based statistics (....) 
%(b) we can show that there exists a convex function ...
%(c) an approximation to it is easily computable
%\end{itemize}

%%%%%%%%SOME STUFF MAY GO ELSEWHERE
%Previous work focuses on proposing new MIAs towards higher advantages.
% The MIA with higher advantage helps with the applications of MIA: 
% it reveals larger privacy vulnerability to motivate the study of privacy-preserving algorithms further; it is a more strict privacy metric when auditing the privacy of any machine learning models.
% We alternatively study the upper bound among a family of MIAs instead of an individual to further enhance the applications.
% In this paper, we focus on score-based MIAs as introduced in Section~\ref{sec:preliminary}.
% We introduce two criteria for choosing the family to fit the applications of MIA.
% By following the criteria, we define a family of score-based MIA whose scores are convex in $(f(x), y)$.
% Because of the inherent complexity of computing the exact upper bound, we derive an approximation algorithm for the upper bound.

%\todo{intro: start from single stats and the application of them. Then we say this motivates the study for a family of MIAs.}
%
%%0: lower bound of advantage. motivates the upper bound. discuss the meaning of the upper bound.
%%1: draw the connection to the discrepancy distance and propose the upper bound.?
%%2: Choose a family -- convex family; Prove 4 probability-based scores are in this family.?
%%3: Introduce how to approximately compute this upper bound.
%While many prior works have been making many towards better MIAs in terms of higher advantage, the upper bound of the advantage among a family of MIAs hasn't gotten much attention yet.
%The upper bound can be useful for two reasons: 1. it is a stronger privacy metric than any single MIA in this family; 2. the comparison between the upper bound and the existing MIAs in the family indicates how good these MIAs are, which can motivate the better design of MIA potentially.
%In this paper, we focus on MIAs which threshold the probability-based scores and we particularly study a family of scores that are convex in $(f(x), y)$. 
%We first show that all four common probability-based scores, as reviewed in Section~\ref{sec:preliminary}, either are in this family or agree on a score in this family.
%As a consequence, the advantages of all four common probability-based scores with arbitrary thresholds are bounded by the upper bound over this family.

% introduces the upper bound over an MIA family

\subsection{Upper Bounds over MIA Families}
\label{sec:gnr_upp}
Suppose $\calM$ is a family of MIAs. For any MIA $m$ in this family, the advantage of $m$ is naturally upper bounded by the maximum advantage among this family, which we denote as ${\rm Adv}(\calM; f, S, \mathcal{D})$:
\begin{equation}
{\rm Adv}(\calM; f, S, \mathcal{D}):= \sup_{m'\in\calM}{\rm Adv}(m'; f, S, \mathcal{D})\geq {\rm Adv}(m; f, S, \mathcal{D}).
\end{equation}
Then ${\rm Adv}(\calM; f, S, \mathcal{D})$ is a more strict privacy metric than the advantage of any single $m\in\calM$.
In this paper, we are particularly interested in a score-based MIA family $\calM_{cvx}$ where the scores are convex or concave in $(f(x), y)$.
The definition of $\calM_{cvx}$ is formally stated as
\begin{equation}
\calM_{cvx}:=\{\mathds{1}\left[h(f, z)< 0\right]|h:\bbR^{2C}\to \bbR \text{ is convex or concave in } (f(x), y)\},\footnote{We omit the threshold $\tau$ because $\mathds{1}\left[h(f, z)< \tau\right]$ $(\forall \tau\in\bbR)$ is indeed contained in $\calM_{cvx}$.
$\mathds{1}\left[h(f, z)< \tau\right]$ is equivalent to $\mathds{1}\left[h(f, z)- \tau<0\right]$ and the convexity are shared between $h(f, z)$  and $h(f, z)-\tau$.}
\end{equation}
where $f(x)\in \bbR^{C}$ is the soft-max probability of the model and $y\in \bbR^{C}$ is the one-hot format label.

We propose ${\rm Adv}(\calM_{cvx}; f, S, \mathcal{D})$ as a better privacy metric for three reasons below.

\textbf{Firstly}, the advantages of a representative set of existing MIAs are bounded by ${\rm Adv}(\calM_{cvx}; f, S, \mathcal{D})$, which ensures ${\rm Adv}(\calM_{cvx}; f, S, \mathcal{D})$ is indeed a better strict privacy metric than the existing MIAs.
We consider four representative score-based MIAs with scores MSP, ENT, CE, and ME\footnote{Check the definitions of these scores in Section~\ref{sec:preliminary}.}; we denote them as $m_{msp, \tau}$, $m_{ent, \tau}$, $m_{ce, \tau}$, and $m_{me, \tau}$ respectively.
The remaining MIAs as reviewed in Section~\ref{sec:preliminary} either are impractical or have no significant merit over them as shown in \citet{watson2021importance, chen2022relaxloss}.
We prove the advantage of these four MIAs are bounded ${\rm Adv}(\calM_{cvx}; f, S, \mathcal{D})$ and state the results in the following theorem.
\begin{theorem}
\label{thm:cvx_up}
	For an arbitrary threshold $\tau\in\bbR$ and any of $m\in\{m_{msp, \tau}, m_{ent, \tau}, m_{ce, \tau}, m_{me, \tau}\}$, 
	$${\rm Adv}(m; f, S, \mathcal{D})\leq {\rm Adv}(\calM_{cvx}; f, S, \mathcal{D}).$$
\end{theorem}
\begin{proof}[Proof sketch of Theorem~\ref{thm:cvx_up}]
	The proof for $m_{msp, \tau}$ and $m_{ent, \tau}$ is straightforward because the MSP score and the ENT score are convex/concave in $(f(x), y)$.
	The proof for $m_{ce, \tau}$ and $m_{me, \tau}$ takes more effort because the cross-entropy score and modified-entropy score are indeed not convex/concave in $(f(x), y)$.
	For each of $m_{ce, \tau}$ and $m_{me, \tau}$, we can construct another function $g(f, z)$ such that 
	\begin{enumerate}
		\item it agrees with the score (CE or ME) for any $(f, z)$;
		\item it is convex or concave in $(f(x), y)$, $\forall$ $f(x), y\in (0, 1]^C\times [0, 1]^C$. 
	\end{enumerate}

	
	This is possible because by definition the label $y$ of $z$ should be a one-hot vector and the convexity is discussed for a larger domain.
	With this construction, ${\rm Adv}(m_{score, \tau}; f, S, \mathcal{D}) = {\rm Adv}(m_{g, \tau}; f, S, \mathcal{D})\leq {\rm Adv}(\calM_{cvx}; f, S, \mathcal{D})$ for $score\in\{ce, me\}$.
\end{proof}
%\begin{remark}
It is worthwhile to highlight from the theorem that ${\rm Adv}(\calM_{cvx}; f, S, \mathcal{D})$ can be proved to be an upper bound for the advantage of an MIA $\mathds{1}\left[h(f(x), y)< 0\right]$ even when $h$ is neither convex nor concave --- the cross-entropy score and modified-entropy score are indeed not convex/concave in $(f(x), y)$.
%\end{remark}

\textbf{Secondly}, ${\rm Adv}(\calM_{cvx}; f, S, \mathcal{D})$ is a non-trivial upper bound and a meaningful privacy metric.
Because the scoring function in $\calM_{cvx}$ is required to be the post-hoc functions of $(f(x), y)$ and further convex/concave in $(f(x), y)$, ${\rm Adv}(\calM_{cvx}; f, S, \mathcal{D})$ is not loose as an upper bound -- we will further show this upper bound is non-vacuous in the later experiment section.
More importantly, as a privacy metric for models, it can be distinguished between different models $f$ -- by contrast, the trivial upper bound ``1'' is not a useful privacy because it cannot tell which model is more privacy-preserving.

\textbf{Lastly}, the approximation of ${\rm Adv}(\calM_{cvx}; f, S, \mathcal{D})$ can be efficiently computed. We show the details in the next section.

%We denote the upper bound as ${\rm Adv}(\calM; f, S, \mathcal{D})$.
%Different from the study of any single MIA, there are two applications to study this upper bound. 
%\begin{enumerate}
%	\item In the context of privacy metrics, MIAs measure the memorization of the model~\citep{nasr2021adversary, steinke2024privacy}. The upper bound is a stronger empirical privacy metric than the advantage of any single MIA in this family.
%	\item As for the study of privacy attacks, the gap between the existing MIA (in this family) and the upper bound motivates to design of a better MIA and further motivates privacy-preserving learning algorithms.
%\end{enumerate} 

\subsection{An Approximation Algorithm for Computing ${\rm Adv}(\calM_{cvx}; f, S, \mathcal{D})$.}
We are going to compute ${\rm Adv}(\calM_{cvx}; f, S, \mathcal{D})$ by showing its equivalence to a parametric optimization problem.
One has proved that the parametric optimization problem is NP-hard.
Therefore, we alternatively smooth the objective function by following \citet{kantchelian2014large} and minimize it by gradient descent to attain an approximate solution.

Firstly, we show the equivalence between ${\rm Adv}(\calM_{cvx}; f, S, \mathcal{D})$ and ${\rm Adv}(\calM_{cvx, k}; f, S, \mathcal{D})$ for some $k\in\bbN$, where we denote $(f(x), y)$ as $a_{f, z}$ for simplicity and define $\calM_{cvx, k}$ as
\begin{align}
\label{eq:cvx_aff}
\calM_{cvx, k}:=\{\mathds{1}\left[s\cdot h(f, z)< 0\right]| & h(f, z):=\max_{i\in[k]}w_i\top a_{f, z}+b_i, w_i\in \bbR^{2C}, b_i\in \bbR, s\in\{1, -1\}\}.
\end{align}
We state this equivalence by the following theorem.
\begin{theorem}
\label{thm:cvx_up2}
	There exists a $k\in\bbN$ such that
	$
	{\rm Adv}(\calM_{cvx, k}; f, S, \mathcal{D}) = {\rm Adv}(\calM_{cvx}; f, S, \mathcal{D}).
	$
\end{theorem}

%
%Now we can rewrite ${\rm Adv}(\calM_{cvx}; f, S, \mathcal{D})$ as
%\begin{equation}
%\label{eq:optim_cpb}
%\max_{w_i\in\bbR^{2C}, b_i\in\bbR, i\in[k], s\in\{1, -1\}}\bbP_{z\sim S}\left(s\cdot \max_{i\in[k]}w_i\top a_{z, f}+b_i<0\right) - \bbP_{z\sim \calD}\left(s\cdot \max_{i\in[k]}w_i\top a_{z, f}+b_i<0\right).
%\end{equation}

Although $\calM_{cvx, k}$ is parametric, finding 
${\rm Adv}(\calM_{cvx, k}; f, S, \mathcal{D})=\sup_{m\in\calM_{cvx, k}}{\rm Adv}(m; f, S, \mathcal{D})$ 
is generally NP-hard even for $k=2$~\cite{gottlieb2018learning}.
Alternatively, by following \citet{kantchelian2014large}, we smooth the objective function by a surrogate classification loss to attain an approximate solution.
We specifically choose logistic regression $\ell_{lg}$.
For each $s\in\{1, -1\}$, the objective function can be written as
$$
\max_{w_i\in\bbR^{2C}, b_i\in\bbR, i\in[k]}
\frac{1}{|S|}\sum_{z\sim S}\ell_{lg}\left(\max_{i\in[k]}w_i\top a_{z, f}+b_i, s\right) + \bbE_{z\sim \calD}\left[\ell_{lg}\left(\max_{i\in[k]}w_i\top a_{z, f}+b_i, -s\right)\right].
$$
Now the objective function is both parametric and continuous.
Although it is still non-convex, we can use gradient descent to find the approximate solution.

To distinguish the exact solution and this approximate solution, we name the maximum advantage over $\calM_{cvx, k}$ the CPB (Convex Polytope Bound) and by following \citet{kantchelian2014large} name the advantage of this approximate solution as the CPM (Convex Polytope Machine).

%Alternatively, we observe that the objective is equivalent to a classification problem and \codo{}
%Similar to \todo{cite}, we instead optimize a smooth surrogate loss 

%Show the reduction to the optimal CPM
%Finding the exact CPM is NP-hard
%Optimize the surrogate instead as an approximation to the upper bound.


%=======================================
\begin{comment}
\subsection{The Choice of the MIA Family -- $\calM_{cvx}$}
\paragraph{Criteria of choosing $\calM$}. We find two criteria of choosing $\calM$ are crucial to the two applications described in Section~\ref{sec:gnr_upp}. 
First, \emph{the family should include as many existing MIAs as possible}. If not, the upper bound of this family is possibly still weaker than the existing MIA not included in this family and both applications are pointless.
Second, \emph{the family can not be arbitrarily large and the upper bound should be achievable}. Otherwise, the upper bound will be loose for any $f, S, D$ and not informative in the first application -- a naive advantage upper bound is $1$ and is not a useful privacy metric in the first application. 
%The larger family also guides the design of MIA weaker in the second application. 

\paragraph{Definition of $\calM_{cvx}$ and criterion validation.} By following the criterion, we propose $\calM_{cvx}$, a family of scoring-based thresholding attack where the scoring function is convex or concave in $(f(x), y)$:
\begin{equation}
\calM_{cvx}:=\{\mathds{1}\left[h(f, z)< 0\right]|h:\bbR^{2C}\to \bbR \text{ is convex or concave in } (f(x), y)\},
\end{equation}
where $f(x)\in \bbR^{C}$ is the soft-max probability of the model and $y\in \bbR^{C}$ is the one-hot format label.

To validate the first criterion, we are going to show the advantages of a sufficient set of existing MIAs are bounded by ${\rm Adv}(\calM_{cvx}; f, S, \mathcal{D})$.
We denote MIAs which threshold the MSP, ENT, CE, and ME as $m_{msp, \tau}$, $m_{ent, \tau}$, $m_{ce, \tau}$, and $m_{me, \tau}$ respectively.
Firstly, it is sufficient to consider these four MIAs\footnote{Check the definitions of these scores in Section~\ref{sec:preliminary}}, because the remaining MIAs as reviewed in Section~\ref{sec:preliminary} either are impractical or has no significant merit over them as shown in the literature~\citep{watson2021importance, chen2022relaxloss}.
Moreover, we can prove the advantage of these four MIAs are bounded ${\rm Adv}(\calM_{cvx}; f, S, \mathcal{D})$ and state the results in the following theorem.

\begin{theorem}
\label{thm:cvx_up}
	For an arbitrary threshold $\tau\in\bbR$ and any of $m\in\{m_{msp, \tau}, m_{ent, \tau}, m_{ce, \tau}, m_{me, \tau}\}$, 
	$${\rm Adv}(m; f, S, \mathcal{D})\leq {\rm Adv}(\calM_{cvx}; f, S, \mathcal{D}).$$
\end{theorem}
\begin{proof}[Proof sketch of Theorem~\ref{thm:cvx_up}]
	The proof for $m_{msp, \tau}$ and $m_{ent, \tau}$ is straightforward because the MSP score and the ENT score are convex/concave in $(f(x), y)$.
	The proof for $m_{ce, \tau}$ and $m_{me, \tau}$ takes more effort because the cross-entropy score and modified-entropy score are indeed not convex/concave in $(f(x), y)$.
	For each of $m_{ce, \tau}$ and $m_{me, \tau}$, we can construct another function $g(f, z)$ such that 
	\begin{enumerate}
		\item it agrees with the score (CE or ME) for any $(f, z)$;
		\item it is convex or concave in $(f(x), y)$, $\forall$ $f(x), y\in (0, 1]^C\times [0, 1]^C$. 
	\end{enumerate}

	
	This is possible because by definition the label $y$ of $z$ should be a one-hot vector and the convexity is discussed for a larger domain.
	With this construction, ${\rm Adv}(m_{score, \tau}; f, S, \mathcal{D}) = {\rm Adv}(m_{g, \tau}; f, S, \mathcal{D})\leq {\rm Adv}(\calM_{cvx}; f, S, \mathcal{D})$ for $score\in\{ce, me\}$.
\end{proof}
\begin{remark}
It is worthwhile to highlight from the theorem that ${\rm Adv}(\calM_{cvx}; f, S, \mathcal{D})$ can be proved to be an upper bound for the advantage of an MIA $\mathds{1}\left[h(f(x), y)< 0\right]$ even when $h$ is neither convex nor convex --- the cross-entropy score and modified-entropy score are indeed not convex/concave in $(f(x), y)$.
\end{remark}

It is straightforward to validate the second criterion. 
By definition, the scoring function is required to be the post-hoc functions of $(f(x), y)$ and further convex/concave in $(f(x), y)$. 
These two constraints together imply a non-trivial upper bound in the first application.
In the second application, these constraints largely shrink the domain to design a scoring function.
\end{comment}
